TESS Observations of Kepler systems with Transit Timing Variations

We identify targets in the Kepler field that may be characterized by transit timing variations (TTVs) and are detectable by the Transiting Exoplanet Survey Satellite (TESS). Despite the reduced signal-to-noise ratio of TESS transits compared to Kepler, we recover 48 transits from 13 systems in Sectors 14, 15, 26, 40 and 41. We find strong evidence of a nontransiting perturber orbiting Kepler-396 (KOI-2672) and explore two possible cases of a third planet in that system that could explain the measured transit times. We update the ephemerides and mass constraints where possible at KOI-70 (Kepler-20), KOI-82 (Kepler-102), KOI-94 (Kepler-89), KOI-137 (Kepler-18), KOI-244 (Kepler-25), KOI-245 (Kepler-37), KOI-282 (Kepler-130), KOI-377 (Kepler-9), KOI-620 (Kepler-51), KOI-806 (Kepler-30), KOI-1353 (Kepler-289) and KOI-1783 (Kepler-1662).

==> trap_table.tex <==
\startlongtable
\begin{deluxetable*}{lcccccc}
\tabletypesize{\tiny}
\tablecaption{Best Fit Trapezoidal Transit Parameters \label{tab:trap}}
\tablehead{
  \colhead{Kepler} &
  \colhead{KOI} &
  \colhead{Sector} &
  \colhead{$T_C$ (BJD$_{\rm TDB}-$2457000)} &
  \colhead{$\delta$ (ppm)} &
  \colhead{$T_{\rm tot}$ (hr)} &
  \colhead{$T_{\rm full}$ (hr)} }
  \startdata
  \multirow{2}{*}{102e} & \multirow{2}{*}{82.01} & 14 & $1697.416^{+0.021}_{-0.029}$ & $940^{+550}_{-460}$ & $3.724^{+0.026}_{-0.025}$ & $3.465\pm0.032$\\
  & & 26 & $2020.3142^{+0.0085}_{-0.018}$ & $590^{+240}_{-250}$ & $3.724\pm0.025$ & $3.466^{+0.031}_{-0.032}$\\
  \hline
  \multirow{5}{*}{65~c} &\multirow{5}{*}{85.01} & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 14 & \nodata & \nodata & \nodata & \nodata \\
  \hline
  \multirow{2}{*}{89A~d} & \multirow{2}{*}{94.01} & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 15 & $1719.3595^{+0.0063}_{-0.0071}$ & $3050\pm370$ & $6.6640\pm0.0039$ & $5.6688^{+0.0056}_{-0.0057}$\\
  \hline
  \multirow{5}{*}{89A~c} &\multirow{5}{*}{94.02} & 14 & $1692.2954^{+0.0091}_{-0.0053}$ & $1620^{+450}_{-470}$ & $5.227\pm0.021$ & $4.922\pm0.020$\\
  & & 14 & $1702.685^{+0.017}_{-0.041}$ & $1590\pm450$ & $5.226\pm0.021$ & $4.921^{+0.020}_{-0.021}$\\
  & & 15 & $1713.098^{+0.035}_{-0.010}$ & $1340^{+410}_{-430}$ & $5.226\pm0.021$ & $4.921\pm0.020$\\
  & & 15 & $1723.569^{+0.041}_{-0.023}$ & $1120^{+470}_{-500}$ & $5.226\pm0.021$ & $4.921\pm0.020$\\
  & & 15 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  89A~e & 94.03 & 14 & $1687.950^{+0.021}_{-0.018}$ & $1740\pm390$ & $8.585\pm0.024$ & $7.783\pm0.028$\\
  \hline
  \multirow{7}{*}{18~c} & \multirow{7}{*}{137.01} & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 15 & $1712.761^{+0.014}_{-0.013}$ & $3400\pm1000$ & $3.4100^{+0.0073}_{-0.0072}$ & $3.118\pm0.013$\\
  & & 15 & \nodata & \nodata & \nodata & \nodata\\
  & & 15 & \nodata & \nodata & \nodata & \nodata\\
  & & 15 & $1735.681^{+0.042}_{-0.016}$ & $3500\pm1000$ & $3.4102^{+0.0073}_{-0.0072}$ & $3.119^{+0.014}_{-0.013}$\\
  \hline
  \multirow{4}{*}{18~d} & \multirow{4}{*}{137.02} & 14 & $1690.7457^{+0.0044}_{-0.0037}$ & $5470\pm760$ & $3.526\pm0.013$ & $3.166\pm0.019$\\
  & & 14 & $1705.6112^{+0.0060}_{-0.0044}$ & $3590^{+780}_{-770}$ & $3.525\pm0.013$ & $3.163\pm0.019$\\
  & & 15 & \nodata & \nodata & \nodata & \nodata\\
  & & 15 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  79~d & 152.01 & 14 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  \multirow{2}{*}{11~e} &\multirow{2}{*}{157.03} & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 15 & \nodata & \nodata & \nodata & \nodata \\
  \hline
  \multirow{2}{*}{122~c} & \multirow{2}{*}{232.01} & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 14 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  \multirow{2}{*}{25A~c} &\multirow{2}{*}{244.01} & 14 & $1687.7126^{+0.0033}_{-0.0025}$ & $1020\pm160$ & $2.723^{+0.051}_{-0.050}$ & $2.44\pm0.12$\\
  & & 14 & $1700.4451^{+0.0038}_{-0.0061}$ & $980\pm160$ & $2.719^{+0.049}_{-0.050}$ & $2.38\pm0.13$\\
  \hline
  \multirow{4}{*}{25A~b} &\multirow{4}{*}{244.02} & 14 & $1685.4358^{+0.017}_{-0.0055}$ & $400^{+150}_{-170}$ & $3.525\pm0.011$ & $3.383\pm0.018$\\
  & & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 14 & $1697.9118^{+0.0061}_{-0.0038}$ & $660\pm150$ & $3.526\pm0.011$ & $3.384^{+0.018}_{-0.017}$\\
  & & 14 & $1704.1262^{+0.0079}_{-0.0092}$ & $700\pm140$ & $3.525\pm0.010$ & $3.383\pm0.017$\\
  \hline
  \multirow{3}{*}{36~c} &\multirow{3}{*}{277.01} & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 15 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  \multirow{2}{*}{9~b} &\multirow{2}{*}{377.01} & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 26 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  \multirow{2}{*}{9~c} &\multirow{2}{*}{377.02} & 14 & \nodata & \nodata & \nodata & \nodata\\
  & & 26 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  149~b & 401.01 & 14 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  51~b & 620.01 & 14 & $1694.879^{+0.021}_{-0.011}$ & $5930\pm960$ & $5.783\pm0.022$ & $4.961^{+0.043}_{-0.042}$\\
  \hline
  51~d & 620.02 & 14 & $1689.996^{+0.023}_{-0.013}$ & $5870\pm880$ & $8.454\pm0.021$ & $6.892^{+0.046}_{-0.047}$\\
  \hline
  30~c & 806.02 & 14 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  82~c & 880.02 & 15 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  \multirow{5}{*}{83A~b} &\multirow{5}{*}{898.01} & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 26 & \nodata & \nodata & \nodata & \nodata \\
  & & 26 & \nodata & \nodata & \nodata & \nodata \\
  & & 26 & \nodata & \nodata & \nodata & \nodata \\
  \hline
  \multirow{2}{*}{83A~c} &\multirow{2}{*}{898.03} & 14 & \nodata & \nodata & \nodata & \nodata \\
  & & 26 & \nodata & \nodata & \nodata & \nodata \\
  \hline
  289~c & 1353.01 & 15 & $1719.730^{+0.012}_{-0.014}$ & $6500^{+880}_{-870}$ & $9.018\pm0.015$ & $7.345\pm0.015$\\
  \hline
  297~c & 1426.02 & 14 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  1662~c & 1783.02 & 15 & \nodata & \nodata & \nodata & \nodata\\
  \hline
  396~c & 2672.01 & 15 & $1733.3103^{+0.0039}_{-0.0064}$ & $2070\pm200$ & $6.808^{+0.087}_{-0.089}$ & $6.12\pm0.11$\\
  \hline
  \multirow{2}{*}{396~b} &\multirow{2}{*}{2672.02} & 14 & $1692.9172^{+0.0069}_{-0.0060}$ & $1310^{+250}_{-240}$ & $4.75\pm0.11$ & $4.17^{+0.37}_{-0.73}$\\
  & & 15 & $1735.887^{+0.047}_{-0.036}$ & $1490^{+260}_{-250}$ & $4.76\pm0.11$ & $4.10^{+0.53}_{-1.1}$\\
  \enddata
\end{deluxetable*}
